Performance of quantum data transmission systems in the presence of thermal noise

In the literature the performance of quantum data transmission systems is usually evaluated in the absence of thermal noise. A more realistic approach taking into account the thermal noise is intrinsically more difficult because it requires dealing with Glauber coherent states in an infinite--dimensional space. In particular, the exact evaluation of the optimal measurement operators is a very difficult task, and numerical approximation is unavoidable. The paper faces the problem by approximating the P-representation of the noisy quantum states with a large but finite number of terms and applying to them the square root measurement (SRM) approach. Comparisons with the exact solution obtained with convex semidefinite programming show that the SRM approach gives quite accurate results. As application, the performance of quadrature amplitude modulation (QAM) and phase shift keying (PSK) systems is considered. In spite of the fact that the SRM approach is not optimal and overestimates the error probability, also in these cases the quantum detection maintains its superiority with respect to the classical homodyne detection.

==> QA/QA114.tex <==
% File: ./CR/CR15.tex creato da CA.m il {2008, 6, 17, 16, 49, 9.703325}
\l=103  \r=90  \unit=0.8mm
 % riga 1 di TeX

\xF=-54 \lD=110
 %\grigliatrue
 \where=2
 % termine di TeX
 \Figura
 DIDASCALIA:Error probability in 8--PSK versus $N_s$ for some
 values of $\C(N)$. Solid lines refer to quantum detection
 and dashed lines to classical homodyne detection.
 INIZIO
\put(0.80,65.41){\BP(102.60,85.30)
\put(-4.648,-81.539){\psfig{figure=./QA/QA114b.ps
,height=88.67mm,width= 129.272mm } }
%
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C1
\w(77,-48)[2,\C(N)=0]\w(94,-13)[2,\C(N)=0]
\w(77.5,-21.7)[2,\C(N)=0.1]
\w(77.5,-13.7)[2,\C(N)=0.2]\w(94.5,-2)[2,\C(N)=0.2]
\w(77.5,-30)[2,\C(N)=0.05]
% termine aggiunte di C1
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 17.1 5,\sx 34.2 10,\sx 51.3 15,\sx 68.4 20,\sx 85.5 25,\sx 102.6 30,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=17.10 n=7
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(94.05,-67.98)(2,c,{{N_s}}\relax)\W(-4.00,15.99)(2,r,{{P_e}}\relax)
 fine
%
 %---------------- Curva N. 2 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C2
% termine aggiunte di C2
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 17.1 5,\sx 34.2 10,\sx 51.3 15,\sx 68.4 20,\sx 85.5 25,\sx 102.6 30,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=17.10 n=7
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(94.05,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 3 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C3
% termine aggiunte di C3
\carattere=2 distanza=65.0
\sx 0.0 0,\sx 17.1 5,\sx 34.2 10,\sx 51.3 15,\sx 68.4 20,\sx 85.5 25,\sx 102.6 30,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=17.10 n=7
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(94.05,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 4 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C4
% termine aggiunte di C4
\carattere=2 distanza=65.0
\sx 0.0 0,\sx 17.1 5,\sx 34.2 10,\sx 51.3 15,\sx 68.4 20,\sx 85.5 25,\sx 102.6 30,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=17.10 n=7
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(94.05,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 5 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C5
% termine aggiunte di C4
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 17.1 5,\sx 34.2 10,\sx 51.3 15,\sx 68.4 20,\sx 85.5 25,\sx 102.6 30,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=17.10 n=7
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=3.42 n=30
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(94.05,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
 \EP}
 FINE


==> QA/QA117.tex <==
% File: ./CR/CR16.tex creato da CA.m il {2008, 6, 17, 18, 15, 48.105355}
\l=103  \r=90  \unit=0.8mm  
 % riga 1 di TeX 
 \lD=110  \xD=0
\xF=-53 \where=2 
% \grigliatrue
                                                    
 % termine di TeX                                                   
 \Figura
 DIDASCALIA:Error probability in 16--QAM versus $N_s$ for some 
 values of $\C(N)$. Solid lines refer to quantum detection
 ans dashed lines to classical homodyne detection.                                                        
 INIZIO
\put(0.80,65.41){\BP(102.60,85.30) 
\put(-4.648,-81.539){\psfig{figure=./QA/QA116.ps ,height=88.67mm,width= 129.272mm } }
% 
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio 
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C1
%new
\WWW[11](78.5,-14)[2,1,\C(N)=0.1\!\!\!]
\WWW[10](71.5,-2)[2,d,\C(N)=0.2] \vet(71.5,8)(67.0,-2)
\WWW[4](66.5,-14)[2,1,\C(N)=0.05]
\circlepath1.5(82,-39)(96,-19)[0.5]\w(84,-28)[2,\C(N)=0]
% termine aggiunte di C1
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 5,\sx 25.6 10,\sx 38.5 15,\sx 51.3 20,\sx 64.1 25,
 \sx 77.0 30,\sx 89.8 35,\sx 102.6 40,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{N_s}}\relax)\W(-4.00,15.99)(2,r,{{P_e}}\relax)
 fine  
% 
 %---------------- Curva N. 2 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio 
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C2
% termine aggiunte di C2
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 5,\sx 25.6 10,\sx 38.5 15,\sx 51.3 20,\sx 64.1 25,
 \sx 77.0 30,\sx 89.8 35,\sx 102.6 40,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine  
% 
 %---------------- Curva N. 3 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio 
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C3
% termine aggiunte di C3 
\carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 5,\sx 25.6 10,\sx 38.5 15,\sx 51.3 20,\sx 64.1 25,
 \sx 77.0 30,\sx 89.8 35,\sx 102.6 40,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine  
% 
 %---------------- Curva N. 4 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio 
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C4
% termine aggiunte di C4
\carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 5,\sx 25.6 10,\sx 38.5 15,\sx 51.3 20,\sx 64.1 25,
 \sx 77.0 30,\sx 89.8 35,\sx 102.6 40,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine  
% 
 %---------------- Curva N. 5 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio 
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C5
% termine aggiunte di C4
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 5,\sx 25.6 10,\sx 38.5 15,\sx 51.3 20,\sx 64.1 25,
 \sx 76.9 30,\sx 89.8 35,\sx 102.6 40,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine  
 \EP} 
 FINE


==> QA/QA2.tex <==
%\l=0\r=11 \rn=0 \xD=40\lD=125\yF=8\yD=10
\def\C(#1){{\cal #1}}
\Z=2  \xF=-8
%\poniombre
%\provatrue 
\unit=0.4mm
\xF=-126
\xD=-110
\where=2
\Blocchi TIPO:\a=10\b=17\c=6\d=13
         NUMERO:2%non importa
DIDASCALIA: Model of a quantum data transmission system.
DOMINI:
FUNZIONI:,a\in\C(A),|\gamma_a\rangle,
             \rho_a,\hat a , ,
SCRITTE:\noS\circoloisolato(15;
          \shortstack{\footnotesize classical\\
	  \footnotesize data\\
	  \footnotesize source}),
\scritta(3)(quantum\\modulator),
        \scritta(3)(quantum\\noisy\\channel),
	\scritta(3)(quantum\\detection),
SOPRASCRITTE:,\scritta(3)(Alice),,\scritta(3)(Bob),
AGGIUNTE:\WWW[12](114,23)[13,d,pure state] \WWW[12](168,23)[13,d,density op.]
FINE







==> QA/QA224.tex <==
% File: ./CR/CR221.tex creato da CA.m il {2008, 6, 30, 6, 42, 50.968969}
\l=120  \r=56  \unit=1.3mm  
 % riga 1 di TeX 
 
\xF=2 \lD=120 \xD=10
% \grigliatrue
                                                    
 % termine di TeX                                                   
 \Figura
 DIDASCALIA:Error probability in 2--PSK and 4--PSK versus $N_s$ for some 
 values of $\C(N)$. The SRM detection is compared with the optimum detection.                                                      
 INIZIO
 \put(2.08,34.44){\BP(54.15,54.21) 
\put(-4.106,-46.824){\psfig{figure=./QA/QA224A.ps ,height=102.118mm,width= 110.872mm } }
% 
 %---------------- Curva N. 1 -------------
\Assi0(-2.075,-31.943) AM=0.000  A=54.150  BM=32.527  B=54.211
inizio 
\W(53.15,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.68)(2,r,{{}}\relax)
% riga 1 di C1
\w(38,17)[10,2--PSK]
%\w(66,-31)[2,\C(N)=0]
\w(48.5,-9)[2,\C(N)=0.2]
\w(48.5,-20)[2,\C(N)=0.1]
%\WWW[5](36,-15)[13,3,\hskip2mmSRM]\WWW[8](36,-12)[13,u,optimum]
\WWW[7](25,0.8)[13,3,SRM]\WWW[8.5](25,-1)[13,u,optimum]\w(25,-14)[13,(Helstrom)]
%\w(66.5,-22)[2,\C(N)=0.05]
% termine aggiunte di C1
 \carattere=2 distanza=33.5
\sx 0.0 0,\sx 10.8 1,\sx 21.7 2,\sx 32.5 3,\sx 43.3 4,\sx 54.2 5,
\tacchex:p=-32.53 h=54.21 s=0.06 o=0.00 d=10.83 n=6
\tacchex:p=-32.53 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\tacchex:p=21.01 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\carattere=2 distanza=1.0
\sy -32.5 10^{-5},\sy -21.7 10^{-4},\sy -10.8 10^{-3},\sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.7 10^{0},
\tacchey:p=0.00 h=54.15 s=0.06 o=-32.53 d=10.84 n=6
\tacchey:p=0.00 h=0.68 s=0.04 o=-29.26 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-29.26 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-26.00 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-26.00 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-24.09 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-24.09 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-22.74 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-22.74 d=10.84 n=5
{\linethickness{0.300\unitlength} \linR(0.00,-32.53,54.15)\linU(0.00,-32.53,54.21)
\linD(54.15,21.68,54.21)\linL(54.15,21.68,54.15)}
\W(48.74,-36.53)(2,c,{{N_s}}\relax)\W(-4.00,16.26)(2,r,{{P_e}}\relax)
 fine  
% 
 %---------------- Curva N. 2 -------------
\Assi0(-2.075,-31.943) AM=0.000  A=54.150  BM=32.527  B=54.211
inizio 
\W(53.15,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.68)(2,r,{{}}\relax)
% riga 1 di C2
% termine aggiunte di C2
 \carattere=2 distanza=33.5
\sx 0.0 0,\sx 10.8 1,\sx 21.7 2,\sx 32.5 3,\sx 43.3 4,\sx 54.2 5,
\tacchex:p=-32.53 h=54.21 s=0.06 o=0.00 d=10.83 n=6
\tacchex:p=-32.53 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\tacchex:p=21.01 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\carattere=2 distanza=1.0
\sy -32.5 10^{-5},\sy -21.7 10^{-4},\sy -10.8 10^{-3},\sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.7 10^{0},
\tacchey:p=0.00 h=54.15 s=0.06 o=-32.53 d=10.84 n=6
\tacchey:p=0.00 h=0.68 s=0.04 o=-29.26 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-29.26 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-26.00 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-26.00 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-24.09 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-24.09 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-22.74 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-22.74 d=10.84 n=5
{\linethickness{0.300\unitlength} \linR(0.00,-32.53,54.15)\linU(0.00,-32.53,54.21)
\linD(54.15,21.68,54.21)\linL(54.15,21.68,54.15)}
\W(48.74,-36.53)(2,c,{{}}\relax)\W(-4.00,16.26)(2,r,{{}}\relax)
 fine  
% 
 %---------------- Curva N. 3 -------------
\Assi0(-2.075,-31.943) AM=0.000  A=54.150  BM=32.527  B=54.211
inizio 
\W(53.15,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.68)(2,r,{{}}\relax)
% riga 1 di C3
% termine aggiunte di C3 
\carattere=2 distanza=33.5
\sx 0.0 0,\sx 10.8 1,\sx 21.7 2,\sx 32.5 3,\sx 43.3 4,\sx 54.2 5,
\tacchex:p=-32.53 h=54.21 s=0.06 o=0.00 d=10.83 n=6
\tacchex:p=-32.53 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\tacchex:p=21.01 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\carattere=2 distanza=1.0
\sy -32.5 10^{-5},\sy -21.7 10^{-4},\sy -10.8 10^{-3},\sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.7 10^{0},
\tacchey:p=0.00 h=54.15 s=0.06 o=-32.53 d=10.84 n=6
\tacchey:p=0.00 h=0.68 s=0.04 o=-29.26 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-29.26 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-26.00 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-26.00 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-24.09 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-24.09 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-22.74 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-22.74 d=10.84 n=5
{\linethickness{0.300\unitlength} \linR(0.00,-32.53,54.15)\linU(0.00,-32.53,54.21)
\linD(54.15,21.68,54.21)\linL(54.15,21.68,54.15)}
\W(48.74,-36.53)(2,c,{{}}\relax)\W(-4.00,16.26)(2,r,{{}}\relax)
 fine  
% 
 %---------------- Curva N. 4 -------------
\Assi0(-2.075,-31.943) AM=0.000  A=54.150  BM=32.527  B=54.211
inizio 
\W(53.15,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.68)(2,r,{{}}\relax)
% riga 1 di C4
% termine aggiunte di C4
 \carattere=2 distanza=33.5
\sx 0.0 0,\sx 10.8 1,\sx 21.7 2,\sx 32.5 3,\sx 43.3 4,\sx 54.2 5,
\tacchex:p=-32.53 h=54.21 s=0.06 o=0.00 d=10.83 n=6
\tacchex:p=-32.53 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\tacchex:p=21.01 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\carattere=2 distanza=1.0
\sy -32.5 10^{-5},\sy -21.7 10^{-4},\sy -10.8 10^{-3},\sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.7 10^{0},
\tacchey:p=0.00 h=54.15 s=0.06 o=-32.53 d=10.84 n=6
\tacchey:p=0.00 h=0.68 s=0.04 o=-29.26 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-29.26 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-26.00 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-26.00 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-24.09 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-24.09 d=10.84 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-22.74 d=10.84 n=5
\tacchey:p=53.47 h=0.68 s=0.04 o=-22.74 d=10.84 n=5
{\linethickness{0.300\unitlength} \linR(0.00,-32.53,54.15)\linU(0.00,-32.53,54.21)
\linD(54.15,21.68,54.21)\linL(54.15,21.68,54.15)}
\W(48.74,-36.53)(2,c,{{}}\relax)\W(-4.00,16.26)(2,r,{{}}\relax)
 fine  
 \EP}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\put(70.08,28.84){\BP(54.15,53.69) 
\put(-4.106,-37.552){\psfig{figure=./QA/QA224B.ps ,height=98.935mm,width= 110.872mm } }
% 
 %---------------- Curva N. 1 -------------
\Assi0(-2.075,-26.344) AM=0.000  A=54.150  BM=26.844  B=53.689
inizio 
\W(53.15,-1.50)(2,t,{{}}\relax)
\W(-1.50,25.84)(2,r,{{}}\relax)
% riga 1 di C1
%\w(66,-31)[2,\C(N)=0]
\w(38,20)[10,4--PSK]
\w(46.5,2)[2,\C(N)=0.4]
\w(46.5,-5)[2,\C(N)=0.2]
\WWW[5](36,5)[13,3,\hskip2mmSRM]\WWW[7](36,3.3)[13,u,optimum]
%\WWW[7](30,3.8)[13,3,SRM]\WWW[8](30,2.3)[13,u,optimum]
%\w(66.5,-22)[2,\C(N)=0.05]
% termine aggiunte di C1
 \carattere=2 distanza=27.8
\sx 0.0 0,\sx 10.8 1,\sx 21.7 2,\sx 32.5 3,\sx 43.3 4,\sx 54.2 5,
\tacchex:p=-26.84 h=53.69 s=0.06 o=0.00 d=10.83 n=6
\tacchex:p=-26.84 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\tacchex:p=26.17 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\carattere=2 distanza=1.0
\sy -26.8 10^{-4},\sy -13.4 10^{-3},\sy 0.0 10^{-2},\sy 13.4 10^{-1},\sy 26.8 10^{0},
\tacchey:p=0.00 h=54.15 s=0.06 o=-26.84 d=13.42 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-22.80 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-22.80 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-18.76 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-18.76 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-16.40 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-16.40 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-14.72 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-14.72 d=13.42 n=4
{\linethickness{0.300\unitlength} \linR(0.00,-26.84,54.15)\linU(0.00,-26.84,53.69)
\linD(54.15,26.84,53.69)\linL(54.15,26.84,54.15)}
\W(48.74,-30.84)(2,c,{{N_s}}\relax)\W(-4.00,20.13)(2,r,{{P_e}}\relax)
 fine  
% 
 %---------------- Curva N. 2 -------------
\Assi0(-2.075,-26.344) AM=0.000  A=54.150  BM=26.844  B=53.689
inizio 
\W(53.15,-1.50)(2,t,{{}}\relax)
\W(-1.50,25.84)(2,r,{{}}\relax)
% riga 1 di C2
% termine aggiunte di C2
 \carattere=2 distanza=27.8
\sx 0.0 0,\sx 10.8 1,\sx 21.7 2,\sx 32.5 3,\sx 43.3 4,\sx 54.2 5,
\tacchex:p=-26.84 h=53.69 s=0.06 o=0.00 d=10.83 n=6
\tacchex:p=-26.84 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\tacchex:p=26.17 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\carattere=2 distanza=1.0
\sy -26.8 10^{-4},\sy -13.4 10^{-3},\sy 0.0 10^{-2},\sy 13.4 10^{-1},\sy 26.8 10^{0},
\tacchey:p=0.00 h=54.15 s=0.06 o=-26.84 d=13.42 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-22.80 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-22.80 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-18.76 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-18.76 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-16.40 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-16.40 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-14.72 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-14.72 d=13.42 n=4
{\linethickness{0.300\unitlength} \linR(0.00,-26.84,54.15)\linU(0.00,-26.84,53.69)
\linD(54.15,26.84,53.69)\linL(54.15,26.84,54.15)}
\W(48.74,-30.84)(2,c,{{}}\relax)\W(-4.00,20.13)(2,r,{{}}\relax)
 fine  
% 
 %---------------- Curva N. 3 -------------
\Assi0(-2.075,-26.344) AM=0.000  A=54.150  BM=26.844  B=53.689
inizio 
\W(53.15,-1.50)(2,t,{{}}\relax)
\W(-1.50,25.84)(2,r,{{}}\relax)
% riga 1 di C3
% termine aggiunte di C3 
\carattere=2 distanza=27.8
\sx 0.0 0,\sx 10.8 1,\sx 21.7 2,\sx 32.5 3,\sx 43.3 4,\sx 54.2 5,
\tacchex:p=-26.84 h=53.69 s=0.06 o=0.00 d=10.83 n=6
\tacchex:p=-26.84 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\tacchex:p=26.17 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\carattere=2 distanza=1.0
\sy -26.8 10^{-4},\sy -13.4 10^{-3},\sy 0.0 10^{-2},\sy 13.4 10^{-1},\sy 26.8 10^{0},
\tacchey:p=0.00 h=54.15 s=0.06 o=-26.84 d=13.42 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-22.80 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-22.80 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-18.76 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-18.76 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-16.40 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-16.40 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-14.72 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-14.72 d=13.42 n=4
{\linethickness{0.300\unitlength} \linR(0.00,-26.84,54.15)\linU(0.00,-26.84,53.69)
\linD(54.15,26.84,53.69)\linL(54.15,26.84,54.15)}
\W(48.74,-30.84)(2,c,{{}}\relax)\W(-4.00,20.13)(2,r,{{}}\relax)
 fine  
% 
 %---------------- Curva N. 4 -------------
\Assi0(-2.075,-26.344) AM=0.000  A=54.150  BM=26.844  B=53.689
inizio 
\W(53.15,-1.50)(2,t,{{}}\relax)
\W(-1.50,25.84)(2,r,{{}}\relax)
% riga 1 di C4
% termine aggiunte di C4
 \carattere=2 distanza=27.8
\sx 0.0 0,\sx 10.8 1,\sx 21.7 2,\sx 32.5 3,\sx 43.3 4,\sx 54.2 5,
\tacchex:p=-26.84 h=53.69 s=0.06 o=0.00 d=10.83 n=6
\tacchex:p=-26.84 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\tacchex:p=26.17 h=0.68 s=0.04 o=0.00 d=2.17 n=25
\carattere=2 distanza=1.0
\sy -26.8 10^{-4},\sy -13.4 10^{-3},\sy 0.0 10^{-2},\sy 13.4 10^{-1},\sy 26.8 10^{0},
\tacchey:p=0.00 h=54.15 s=0.06 o=-26.84 d=13.42 n=5
\tacchey:p=0.00 h=0.68 s=0.04 o=-22.80 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-22.80 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-18.76 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-18.76 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-16.40 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-16.40 d=13.42 n=4
\tacchey:p=0.00 h=0.68 s=0.04 o=-14.72 d=13.42 n=4
\tacchey:p=53.47 h=0.68 s=0.04 o=-14.72 d=13.42 n=4
{\linethickness{0.300\unitlength} \linR(0.00,-26.84,54.15)\linU(0.00,-26.84,53.69)
\linD(54.15,26.84,53.69)\linL(54.15,26.84,54.15)}
\W(48.74,-30.84)(2,c,{{}}\relax)\W(-4.00,20.13)(2,r,{{}}\relax)
 fine  
 \EP} 
 FINE


==> QA/QA310.tex <==
% File: ./CR/CR14.tex creato da CA.m il {2008, 6, 20, 10, 56, 45.244596}
\l=103  \r=91  \unit=0.8mm
 % riga 1 di TeX

\xF=-53  \lD=110
% \grigliatrue
\where=2
 % termine di TeX
 \Figura
 DIDASCALIA:Error probability in 4--PSK versus $N_s$ for some
 values of $\C(N)$. Solid lines refer to quantum detection
 and dashed lines to classical homodyne detection.
 INIZIO
\put(0.80,68.72){\BP(102.60,86.25)
\put(-4.648,-88.119){\psfig{figure=./QA/QA310b.ps
,height=91.76mm,width= 129.272mm } }
%
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-66.222) AM=0.000  A=102.600  BM=67.080  B=86.246
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,18.17)(2,r,{{}}\relax)
% riga 1 di C1
\w(77,-36)[2,\C(N)=0]
\WWW[7](50.5,-8)[2,1,\C(N)=0.1\!\!\!]
\WWW[10](66.5,-6)[2,d,\C(N)=0.2] \vet(66.5,4)(62.0,-7)
\WWW[4](66.5,-22)[2,1,\C(N)=0.05]
\circlepath1.5(75,-44)(92,-25)[0.5]
% termine aggiunte di C1
 \carattere=2 distanza=68.1
\sx 0.0 0,\sx 10.3 1,\sx 20.5 2,\sx 30.8 3,\sx 41.0 4,\sx 51.3 5,
 \sx 61.6 6,\sx 71.8 7,\sx 82.1 8,\sx 92.3 9,\sx 102.6 10,
\tacchex:p=-67.08 h=86.25 s=0.06 o=0.00 d=10.26 n=11
\tacchex:p=-67.08 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\tacchex:p=17.88 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\carattere=2 distanza=1.0
\sy -67.1 10^{-9},\sy -57.5 10^{-8},\sy -47.9 10^{-7},\sy -38.3 10^{-6},\sy -28.7 10^{-5},\sy -19.2 10^{-4},
 \sy -9.6 10^{-3},\sy 0.0 10^{-2},\sy 9.6 10^{-1},\sy 19.2 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-67.08 d=9.58 n=10
\tacchey:p=0.00 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
{\linethickness{0.300\unitlength} \linR(0.00,-67.08,102.60)\linU(0.00,-67.08,86.25)
\linD(102.60,19.17,86.25)\linL(102.60,19.17,102.60)}
\W(97.47,-71.08)(2,c,{{N_s}}\relax)\W(-4.00,14.37)(2,r,{{P_e}}\relax)
 fine
%
 %---------------- Curva N. 2 -------------
\Assi0(-0.800,-66.222) AM=0.000  A=102.600  BM=67.080  B=86.246
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,18.17)(2,r,{{}}\relax)
% riga 1 di C2
% termine aggiunte di C2
 \carattere=2 distanza=68.1
\sx 0.0 0,\sx 10.3 1,\sx 20.5 2,\sx 30.8 3,\sx 41.0 4,\sx 51.3 5,
 \sx 61.6 6,\sx 71.8 7,\sx 82.1 8,\sx 92.3 9,\sx 102.6 10,
\tacchex:p=-67.08 h=86.25 s=0.06 o=0.00 d=10.26 n=11
\tacchex:p=-67.08 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\tacchex:p=17.88 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\carattere=2 distanza=1.0
\sy -67.1 10^{-9},\sy -57.5 10^{-8},\sy -47.9 10^{-7},\sy -38.3 10^{-6},\sy -28.7 10^{-5},\sy -19.2 10^{-4},
 \sy -9.6 10^{-3},\sy 0.0 10^{-2},\sy 9.6 10^{-1},\sy 19.2 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-67.08 d=9.58 n=10
\tacchey:p=0.00 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
{\linethickness{0.300\unitlength} \linR(0.00,-67.08,102.60)\linU(0.00,-67.08,86.25)
\linD(102.60,19.17,86.25)\linL(102.60,19.17,102.60)}
\W(97.47,-71.08)(2,c,{{}}\relax)\W(-4.00,14.37)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 3 -------------
\Assi0(-0.800,-66.222) AM=0.000  A=102.600  BM=67.080  B=86.246
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,18.17)(2,r,{{}}\relax)
% riga 1 di C3
% termine aggiunte di C3
\carattere=2 distanza=68.1
\sx 0.0 0,\sx 10.3 1,\sx 20.5 2,\sx 30.8 3,\sx 41.0 4,\sx 51.3 5,
 \sx 61.6 6,\sx 71.8 7,\sx 82.1 8,\sx 92.3 9,\sx 102.6 10,
\tacchex:p=-67.08 h=86.25 s=0.06 o=0.00 d=10.26 n=11
\tacchex:p=-67.08 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\tacchex:p=17.88 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\carattere=2 distanza=1.0
\sy -67.1 10^{-9},\sy -57.5 10^{-8},\sy -47.9 10^{-7},\sy -38.3 10^{-6},\sy -28.7 10^{-5},\sy -19.2 10^{-4},
 \sy -9.6 10^{-3},\sy 0.0 10^{-2},\sy 9.6 10^{-1},\sy 19.2 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-67.08 d=9.58 n=10
\tacchey:p=0.00 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
{\linethickness{0.300\unitlength} \linR(0.00,-67.08,102.60)\linU(0.00,-67.08,86.25)
\linD(102.60,19.17,86.25)\linL(102.60,19.17,102.60)}
\W(97.47,-71.08)(2,c,{{}}\relax)\W(-4.00,14.37)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 4 -------------
\Assi0(-0.800,-66.222) AM=0.000  A=102.600  BM=67.080  B=86.246
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,18.17)(2,r,{{}}\relax)
% riga 1 di C4
% termine aggiunte di C4
\carattere=2 distanza=68.1
\sx 0.0 0,\sx 10.3 1,\sx 20.5 2,\sx 30.8 3,\sx 41.0 4,\sx 51.3 5,
 \sx 61.6 6,\sx 71.8 7,\sx 82.1 8,\sx 92.3 9,\sx 102.6 10,
\tacchex:p=-67.08 h=86.25 s=0.06 o=0.00 d=10.26 n=11
\tacchex:p=-67.08 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\tacchex:p=17.88 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\carattere=2 distanza=1.0
\sy -67.1 10^{-9},\sy -57.5 10^{-8},\sy -47.9 10^{-7},\sy -38.3 10^{-6},\sy -28.7 10^{-5},\sy -19.2 10^{-4},
 \sy -9.6 10^{-3},\sy 0.0 10^{-2},\sy 9.6 10^{-1},\sy 19.2 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-67.08 d=9.58 n=10
\tacchey:p=0.00 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
{\linethickness{0.300\unitlength} \linR(0.00,-67.08,102.60)\linU(0.00,-67.08,86.25)
\linD(102.60,19.17,86.25)\linL(102.60,19.17,102.60)}
\W(97.47,-71.08)(2,c,{{}}\relax)\W(-4.00,14.37)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 5 -------------
\Assi0(-0.800,-66.222) AM=0.000  A=102.600  BM=67.080  B=86.246
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,18.17)(2,r,{{}}\relax)
% riga 1 di C5
% termine aggiunte di C4
 \carattere=2 distanza=68.1
\sx 0.0 0,\sx 10.3 1,\sx 20.5 2,\sx 30.8 3,\sx 41.0 4,\sx 51.3 5,
 \sx 61.6 6,\sx 71.8 7,\sx 82.1 8,\sx 92.3 9,\sx 102.6 10,
\tacchex:p=-67.08 h=86.25 s=0.06 o=0.00 d=10.26 n=11
\tacchex:p=-67.08 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\tacchex:p=17.88 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\carattere=2 distanza=1.0
\sy -67.1 10^{-9},\sy -57.5 10^{-8},\sy -47.9 10^{-7},\sy -38.3 10^{-6},\sy -28.7 10^{-5},\sy -19.2 10^{-4},
 \sy -9.6 10^{-3},\sy 0.0 10^{-2},\sy 9.6 10^{-1},\sy 19.2 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-67.08 d=9.58 n=10
\tacchey:p=0.00 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-64.20 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.31 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-59.62 d=9.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.43 d=9.58 n=9
{\linethickness{0.300\unitlength} \linR(0.00,-67.08,102.60)\linU(0.00,-67.08,86.25)
\linD(102.60,19.17,86.25)\linL(102.60,19.17,102.60)}
\W(97.47,-71.08)(2,c,{{}}\relax)\W(-4.00,14.37)(2,r,{{}}\relax)
 fine
 \EP}
 FINE


==> QA/TQA4.tex <==
\def\arraystretch{1.8}
\xD=-4\yD=0\lD=110\xF=28\yF=0
\unit=1mm
\def\acapo{\\ \hline}
\def\B(#1){#1}  \def\BB(#1){#1}
\def\Tr{\hb{Tr}}
\begin{footnotesize}
\tabella
DIDASCALIA: Values of $N_\epsilon$ and $N_\nu$ of the dimensions of
state factors for some values of the average number of photons $N_\gamma$
and of the thermal noise parameter $\C(N)$. 
INCOLONNAMENTO:{|c|rr|rr|rr|rr|rr|rr|}
INIZIO
%<<<<<<<<<<<<<<<<<< TITOLI COLONNE {T1,T2}>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>
\hline
 $N_\gamma\arr$ 
   &\multicolumn{2}{|c|}{$0.5$}
   &\multicolumn{2}{|c|}{$1.0$}
   &\multicolumn{2}{|c|}{$5$} 
   &\multicolumn{2}{|c|}{$10$}
   &\multicolumn{2}{|c|}{$15$}
   &\multicolumn{2}{|c|}{$25$}\cr
   \hline
   &$N_\epsilon$&$N_\nu$
   &$N_\epsilon$&$N_\nu$
   &$N_\epsilon$&$N_\nu$
   &$N_\epsilon$&$N_\nu$
   &$N_\epsilon$&$N_\nu$&
   $N_\epsilon$&$N_\nu$\cr
		\hline
$\C(N)=0.001$&7 & 2 &
10 & 2 &
21 & 2 &
31 & 2 &
40 & 2 &
57 & 2\cr
$\C(N)=0.01$&7 & 3 &
9 & 3 &
20 & 2 &
30 & 2 &
39 & 2 &
55 & 2\cr
$\C(N)=0.1$&9 & 4 &
11 & 4 &
22 & 4 &
32 & 4 &
41 & 4 &
57 & 4\cr
$\C(N)=1.0$&21 & 12 &
24 & 12 &
38 & 11 &
51 & 11 &
62 & 10 &
81 & 10\cr
$\C(N)=2.0$&33 & 18 &
36 & 18 &
52 & 17 &
66 & 17 &
78 & 16 &
99 & 16\cr
$\C(N)=3.0$&45 & 24 &
49 & 24 &
67 & 23 &
83 & 22 &
97 & 21 &
121 & 20\cr
\hline
FINE
\end{footnotesize}



==> bqf.tex <==

\begin{small}

\Bibliografario(BB){References}


%[6]
\indent\J(Ban1997) M. Ban, K. Kurokawa, R. Momose, and O. Hirota, ``Optimum
measurements for discrimination among symmetric quantum state and
parameter estimation'', {\it Int. J. Theor. Phys.}, vol. 36, pp.
1269--1288, 1997.


\J(Chefles) A. Chefles, ``Quantum State Discrimination'',
 {\it Contemporary Physics}, vol. 41, pp. 401--424, 2000.
 


\J(JPLbook) S. J. Dolinar, J. Hamkins, B. E. Moiston and  V. A. Vilnrotter,
 ``Optical Modulation and Coding'' in H. Hemmati (Ed),
 {\it Deep Space Optical Communications}. New York: Wiley, 2006.


%[7]
\J(Forney1) Y. C. Eldar and G. D. Forney, Jr., ``On quantum detection and
the square--root measurement'', {\it IEEE Trans. Inform. Theory},
vol IT--47, pp. 858--872, Mar. 2001.

%[5]
\J(Eldar2003)  Y. C. Eldar, A. Megretski, and G. C. Verghese, ``Designing
optimal quantum detectors via semidefinite programming'', {\it
IEEE Trans. Inform. Theory}, vol IT--49, pp. 1007--1012, Apr.
2003.

%[9]
\J(Eldar3)  Y. C. Eldar, A. Megretski, and G. C. Verghese, ``Optimal
detection of symmetric mixed quantum states'', {\it IEEE Trans. Inform. Theory}, 
vol IT--50, pp. 1198--1207, June 2004.


%[10]
\J(Glauber) R. J. Glauber, ``Coherent and incoherent states of the
radiation field'', {\it Phys. Rev.}, vol. 131, pp. 2766--2788, Sep.
1963.

%[8]
\J(Hauslanden) P. Hausladen, R. Josza, B. Schumacher, M. Westmoreland, and
W. K. Wootters, ``Classical information capacity of a quantum
channel'', {\it Phys. Rev. A}, vol. 54, pp. 1869--1876, Sept. 1996.


%[14]
\J(Helstrom) C.W. Helstrom, J.W.S. Liu, and J.P. Gordon, ``Quantum mechanical
communication theory'', {\it Proceedings of the IEEE}, vol. 58, no.
10, pp. 1578--1598, Oct. 1970.

%[1]
\J(Helstrom2) C. W. Helstrom. {\it Quantum Detection and Estimation Theory}.
New York: Academic Press, 1976.



%[2]
\J(Holevo) A. S. Holevo, ``Statistical decision theory for quantum systems'',
{\it J. Multivar. Anal.}, vol. 3, pp. 337--394, Dec. 1973.


\J(Kato1999) K. Kato, M. Osaki, M. Sasaki, and O. Hirota, ``Quantum
detection and mutual information for QAM and PSK signals'', {\it
IEEE Trans. on Commun.}, vol. COM--47, pp. 248--254, Feb. 1999.

%[11]
\J(Sasaki) M. Sasaki, R. Momosek. Kato and O. Hirota, ``Quantum
detection for an on--off keyed mixed--state signal with a small amount of
thermal noise'', {\it Phys. Rev. A}, vol. 55, pp. 3223--3226, April 1997.




%[12]
\J(Vilrotter) V. A. Vilnrotter and C.--W. Lau, ``Quantum detection of binary
and ternary signals in the presence of thermal noise fields'', The
Interplanetary Network Progress Report No. 42--152, Feb. 2003.


%[3]
\J(Yuen) H. P. Yuen, R. S. Kennedy, and M. Lax, ``Optimum testing of
multiple hypotheses in quantum detection theory'', {\it IEEE
Trans. Inform. Theory}, vol IT--21, pp. 125--134, Mar. 1975.

\end{small}


==> qf1.tex <==

\def\B(#1){#1}\def\BB(#1){#1}
\def\Tr{\hb{Tr}}

\def\bk(#1,#2){\langle#1|#2\rangle}
\def\bok(#1,#2,#3){\langle#1|#2|#3\rangle}
\def\kb(#1,#2){|#1\rangle\langle#2|}
\def\lb{\lambda}
\def\ket(#1){|#1\rangle}
\def\mod{\ {\rm mod}\ }
\bozzefalse \setcounter{page}{1}

\begin{abstract}
In the  literature the performance of
quantum data transmission systems is usually evaluated in the
absence of thermal noise. A more realistic approach taking into account the
thermal noise is intrinsically more difficult because it requires dealing
with Glauber coherent states in an infinite--dimensional space. In particular, the
exact evaluation of the optimal measurement operators
 is a very difficult task, and numerical approximation is unavoidable. The paper
 faces the problem by approximating the $P$--representation of the noisy
 quantum states with a large but finite numbers of terms and
applying to them the square root measurement (SRM) approach. Comparisons
 with cases where the exact solution are known show that  the SRM approach
 gives quite accurate results.
  As application, the performance of quadrature amplitude modulation (QAM) and phase shift keying (PSK) systems is considered.
 In spite of the fact that the SRM approach is not optimal and overestimates  the
 error probability, also in these cases the quantum detection maintains its
 superiority with respect to the classical homodyne detection.
\end{abstract}
\vspace{3mm}
\begin{keywords} Quantum detection, square root measurement, geometrically
uniform states, thermal noise, quadrature amplitude modulation (QAM), phase shift keying (PSK).
\end{keywords}

\Paragrafo(IN){Introduction}

Transmission of information through a quantum channel
is mainly affected by an uncertainty which is intrinsically
related to the quantum mechanics laws. In the language of
classical optical systems, this uncertainty corresponds to the
so called {\it shot noise}. Another reason of uncertainty is the
presence of {\it thermal noise}, as in classical systems.
Beginning from 1970's, a
lot of research work has been devoted to the {\it quantum
detection problem} \bibl(Helstrom2), that may be summarized in the
following terms. The transmitter sends a quantum signal through a
quantum channel, which forces the receiver to assume one among a
finite number of states. The detector tries to guess the state by
an adequate set of quantum measurements and the problem arises of
finding the measurement set which optimizes the detection,
according to some predefined fidelity criterion (usually the
minimum error probability). Necessary and sufficient conditions
for the optimal measurement set have been found in pioneering
papers by Holevo \bibl(Holevo) and by Yuen {\it et al.} \bibl(Yuen).

Unfortunately, even though the optimal measurement set is
completely characterized, analytical closed--form solutions for
the measurement set, indeed for the minimum error probability, are
not available, in general. Then, it is needed to resort to a
numerical evaluation based on convex semidefinite programming \bibl(Eldar3).
However, under some rotation symmetry constraint,
a simple measurement, introduced by Hausladen {\it et al.}
\bibl(Hauslanden)  and known as {\it
square root measurement} (SRM), turns out to be optimum. The SRM has
the  remarkable advantage that it is straightforwardly
evaluated starting from the possible states. Moreover,
 also when
it is not optimal, the SRM  often gives ``pretty good'' upper bounds on
the performance of optimal detectors.




Our paper starts just from these important results on SRM for
studying quantum data transmission systems in the presence of
thermal noise. After the pioneering work in \bibl(Helstrom2), the
problem of quantum detection in a noisy environment has received
scarce  attention in the literature. To the best of our
knowledge, only a correspondence by Sasaki {\it et al.} \bibl(Sasaki)
on quantum on--off keying (OOK) and a technical report \bibl(Vilrotter) on quantum
PSK attempt to afford an approximate analysis of quantum detection of
coherent states. This delay is due to the difficulties of performing
efficient approximations in the numerical performance evaluation.
 On the other hand, exploiting the new perspectives
open by the extension of the SRM to mixed states \bibl(Eldar3), we
apply this approach to a quantum noisy channel according to the
Glauber theory on coherent states.


 The paper is organized as follows. In Section II we review
 quantum detection fundamentals. In Sections III the SRM
 techniques
 are recalled and  in Section IV the key problem of the  finite-dimensional
 factorization of the Glauber representation of noisy states is discussed.
 Finally, in Sections V and VI  the SRM approach is applied to
  QAM and PSK quantum systems (the same systems considered
 by Kato {\it et al.} \bibl(Kato1999)  in the absence of thermal noise).


\vspace*{-3mm}

\Paragrafo(QA){ Quantum Data Transmission System}


In this section we recall some basic facts about quantum
detection following the scheme of \Figg(QA2)0. For a detailed treatment the reader
is referred to \bibl(Helstrom2) and for a more recent survey to
\bibl(Chefles).\Figg(QA2)2

\vspace*{-3mm}

\subsection{General Model}

A classical source emits a symbol $a$ drawn from a finite
alphabet $\C(A)=\{0,1,\ldots,m-1\}$ with a
given {\it  prior probability distribution}
$
q_i=\P[a=i]\vl i=0,\ldots,m-1
$.
On the basis of the symbol $a$ emitted by
the source, the transmitter sends a quantum state $\ket(\gamma_a)$
through a
quantum channel (e.g., a laser pulse through an optical fiber). As
a consequence, the  received state  is one of
$m$ possible quantum states and  the detection device performs
a set of measurements in order to guess the received state and
consequently the original symbol.

In the ideal case, i.e. neglecting thermal noise,
a set of $m$ pure states is seen by the receiver, which are  a replica of the
transmitted states $\ket(\gamma_a)$. In the presence of thermal noise
the received states
become noisy (or mixed) and are described by a set of
 {\it density operators}
$\rho_i$, $i=0,\ldots,m-1$, which are Hermitian,
 positive semidefinite (PSD)
and have unit trace, $\Tr(\rho_i)=1$. The description through density operators represents
 the general case, since it is comprehensive of the pure state case,
 in which
 $\rho_i$ reduces to the rank--one
operator
$
\rho_i=\kb(\gamma_i,\gamma_i)
$.



\subsection{ Quantum Detection Theory. Available Results.}

Quantum theory postulates that a detection device for choosing
among the possible states is given by a {\it positive operator
valued measurement} (POVM), i.e. a set of $m$ operators
$\Pi_0,\ldots,\Pi_{m-1}$ that are Hermitian,  PSD
 and resolve the identity operator of the  Hilbert space
$\C(H)$, namely
$
\sum_{i=0}^{m-1}\Pi_i=I_{\C(H)}
$.
Then, the probability that the detection
system reveals the state $j$, provided that the state density
operator is $\rho_i$, is given by
$$
p(j|i)=\Tr(\rho_i\Pi_j)\vq i,j=0,\ldots,m-1\;.
\e(Q4)
$$
In particular, the probability of
correct detection becomes
$$
P_c=\sum_{i=0}^{m-1}q_i\,p(i|i)=\sum_{i=0}^{m-1}q_i\,\Tr(\rho_i\Pi_i)\;.
\e(Q5)
$$
For pure states, that is with $\rho_i=|\gamma_i\rangle\langle\gamma_i|$,
rank--one POVMs of the form $\Pi_j=|\mu_j\rangle\langle\mu_j|$
can be used, where $|\mu_j\rangle$ are called {{\co measurement vectors}. Then,
 \e(Q4) reduces to $p(j|i)=|\bk(\gamma_i,\mu_j)|^2$.


The optimization of the detection scheme reduces to
finding the POVM operators $\Pi_i$ that maximize
$
J=\sum_{i=0}^{m-1}\Tr(q_i\rho_i\Pi_i)
$
under the constraints that the
$\Pi_i$ are PSD and resolve the identity $I_{\C(H)}$.
The maximum of $J$ is the optimal probability of correct
detection. Clearly, this is a convex semidefinite programming
problem in the real space of the Hermitian operators.

On the other hand, analytical closed--form results are available only for
the particular class of pure states exhibiting the so called {\co geometrically
uniform symmetry} (GUS). In this case Ban {\it et al.} \bibl(Ban1997) have
shown that the optimal
POVMs  are given by the SRM. This
 particular solution
has been thoroughly discussed by Eldar and Forney \bibl(Forney1). Recently
the SRM approach has been extended to mixed states
by Eldar {\it et al.} \bibl(Eldar3).




\vspace*{-3mm}

\Paragrafo(SRM){The SRM Techniques}

In this section we review the SRM techniques, having in mind that our final
application will be the optical quantum transmissions, where quantum states
and density operators should be formulated according to the Glauber theory (see
Section IV). The SRM technique is here considered in the  general case of
mixed states, following  Eldar, Megretski  and Verghese \bibl(Eldar3).



\subsection{General Formulation}


We start from a constellation of $m$ density operators $\rho_0,\ldots,\rho_{m-1}$ in an
$n$--dimensional Hilbert space $\C(H)$. The key of the SRM approach
is the factorization of each density operator in the form
$\rho_i=\gamma_i\,\gamma_i^*$
for some complex matrices $\gamma_i$, e.g., via the
eigendecomposition of $\rho_i$.  The factorization is not
unique, but the ambiguity is irrelevant for the quantum decision. If $\rho_i$
has rank $r_i\leq n$, the factor $\gamma_i$ can be chosen to have dimensions
$n\times r_i$. In \bibl(Eldar3) $\gamma_i$ is referred as a factor of $\rho_i$,
but, more specifically,
 we call $\gamma_i$ a {\it state factor}. Since
 the $i$-th optimal measurement operator can be chosen with
rank not greater than the rank of $\rho_i$ \bibl(Eldar2003), the search
can be confined to POVMs of the form
$
\Pi_i= \mu_i\,\mu_i^*
$
where $\mu_i$ are $n\times r_i$ complex matrices. We refer to $\mu_i$ as
{\it measurement factors}.

The (generalized) {\co state}  and the {\co measurement matrices} are obtained by
storing the corresponding $n\times r_i$ factors as block--column vectors,
namely
$
  \Gamma=[\gamma_0,\gamma_1,\ldots, \gamma_{m-1}]$ and
 $ M=[\mu_0,\mu_1,\ldots, \mu_{m-1}]
  $.
The dimensions of both $\Gamma$ and $M$  are  $n\times k$ with
$k=r_0+\cdots+ r_{m-1}$.

  From the state matrix $\Gamma$ we form the $k\times k$ Gram matrix
  $G=\Gamma^*\,\Gamma$
and also the  $n\times n$ matrix
  $T=\Gamma\,\Gamma^*$,
sometimes called Gram operator.

  At this point the SRM method is used to provide
   the measurement matrix $M$. The
  first step is the eigendecompositions  of $G$ and $T$,
  namely $\B(G)=\B(V)\BB(\Lambda)_G\B(V)^*$, $\B(T)=\B(U)\BB(\Lambda)_T\B(U)^*$,
  where  $U$, $V$ are unitary and $\Lambda_G$,  $\Lambda_T$ are diagonal.
  Note that
   $G$ and $T$ are both
  PSD with the same rank $r$ and have the same set
  of positive eigenvalues \bibl(Forney1).
  From the eigendecompositions we can find
 the inverse of the square root of $G$ and $T$ as
$
 G^{-1/2}=V\,\Lambda_G^{-1/2}\,V^*$ and
     $T^{-1/2}=U\,\Lambda_T^{-1/2}\,U^*$,
where the inverses  must be intended in
the generalized Moore--Penrose sense \bibl(Forney1).  Finally,
     the measurement  matrix is given by
$
   M=T^{-1/2}\,\Gamma
     $.

     An alternative evaluation of $M$
 is obtained through the Gram
matrix. In fact, it can be shown \bibl(Forney1) using the singular--value
decomposition, that the measurement matrix is also given by
$
M=\Gamma\,G^{-1/2}
$.
Then, the evaluation of the transition probabilities follows from \e(Q4), namely
$$\eqalign{
p(j|i)=&\Tr(\rho_i\Pi_j)=\Tr(\gamma_i\gamma_i^*\mu_j\mu_j^*)\cr
=&\Tr(\mu_j^*\gamma_i\gamma_i^*\mu_j)=\Tr(B_{ji}B_{ji}^*)\cr}\e(B31)
$$
where $B_{ji}$ is the $(j,i)$--th block of the matrix
$
M^*\Gamma=G^{-1/2}\Gamma^*\Gamma=G^{1/2}
$.
Then, for the evaluation of $p(j|i)$ we have to partition $G^{1/2}$ into blocks.
Finally, the probability of correct decision becomes
$$
P_c={1\over m}\sum_{i=0}^{m-1}\Tr(B_{ii}^*B_{ii})\,.
$$

 This twofold possibility,
via $T^{-1/2}$ or $G^{\pm1/2}$,  is very important for an efficient
computation,
particularly when $k<n$.


\subsection{ SRM with Geometrically
              Uniform Symmetry}

The SRM is simplified and provides peculiar properties if the state constellation
 exhibits the  {\co geometrically uniform symmetry} (GUS), that  is
if there exists a unitary operator%
  \footnote{The GUS can be generalized over a group of unitary operators \bibl(Eldar3),
         but in our applications this generalization is not needed.}
$S$, such that $S^m=I_\C(H)$ and
$
\rho_i=S^i\rho_0S^{-i}
$.
The operator $S$ and the density operator $\rho_0$ are said
the {\it generating operator} and the {\it generating density} of
the constellation, respectively. For the mixed states the factorization $\rho_0=\gamma_0\gamma_0^*$
leads to the form $\gamma_i=S^i\gamma_0$.
Note that with GUS all the state factors $\gamma_i$ have the same rank $h$ as
$\gamma_0$.

Since  $S$ is unitary, its
eigendecomposition has the form
$
S=Y\Lambda Y^*=\sum_{j=0}^{n-1}\lb_j\kb(y_j,y_j)
$,
where $Y$ is a unitary matrix of order $n$ and the eigenvalues
$\lambda_j$ collected in the diagonal matrix $\Lambda$ have unit amplitude. Moreover,
because of $S^m=I_{\C(H)} $, the diagonal matrix has the form
$
\Lambda=\diag\left[W_m^{r_0},\ldots,W_m^{r_{n-1}}\right]
$
where $W_m=e^{i2\pi/m}$ and the exponents $r_i$ are suitable
integers with $0\le r_i<m$. By collecting  the terms with equal
eigenvalues in the eigendecomposition, one gets
$
S=\sum_{k=0}^{m-1}W_m^kY_k
$,
where $Y_k$ are projector operators, so that $Y_hY_k=Y_h\delta_{hk}$.

The Gram matrix $G=\Gamma^*\Gamma$, of order $mh$, is formed by the blocks
 of order $h$
$$\eqalign{
G_{rs}&=\gamma_r^*\gamma_s=\gamma_0^*S^{s-r}\gamma_0\cr
&=\sum_{k=0}^{m-1}W_m^{k(s-r)}\gamma_0^*Y_k\gamma_0=
{1\over m}\sum_{k=0}^{m-1}W_m^{k(s-r)}D_k\;,\cr}
$$
where $D_k=m\gamma_0^*\,Y_k\,\gamma_0$. Since $G_{rs}$ depends only on the difference
$r-s$ mod $m$ the Gram matrix is {\co block circulant}. But,  the important point
is that this property yields an explicit decomposition for $G$, namely
$$
G=V_{m,h}DV_{m,h}^*
\e(P10C)
$$
where $D=\diag\{D_0,\ldots,D_{m-1}\}$ and $V_{m,h}$ is the $hm\times hm$
matrix
$
V_{m,h}=\left|\left|(1/\sqrt m)W_m^{rs}I_h\right|\right|
$
with $I_h$ identity matrix of order $h$. As a consequence,
the diagonal blocks of the matrix are given by the Discrete Fourier Transform (DFT)
 of the first ``block  row''
 of the Gram matrix $G$, namely
$
D_i=\sum_{s=0}^{m-1}G_{0s}W_m^{-is}
$.

Note that \e(P10C) is not a standard eigendecomposition because the blocks
$D_i$ are not diagonal matrices. To find the square root of $G$
we have to evaluate the square root of $D$ with an eigendecomposition
of each block $D_i$. Since these are PSD Hermitian square matrices,
their square roots matrices $D_i^{\pm 1/2}$  can be calculated
to construct
$D^{\pm1/2}=\diag[D_0^{\pm1/2},\ldots,D_{m-1}^{\pm1/2}]$. Finally, we obtain
  $
G^{\pm1/2}=V_{m,h}\,D^{\pm1/2}\,V_{m,h}^*
$
whose $(r,s)$ block
is given by
$$
[\,G^{\pm1/2}\,]_{rs}=\frac{1}{\sqrt{m}}\
          \sum_{i=0}^{m-1}W_m^{(s-r)i}D_i^{\pm1/2}\;.
      \e(P35)
$$

Now, the  probabilities $p(j|i)$ are obtained
by applying \e(B31) with $B_{ji}=(G^{1/2})_{ji}$. In particular,
$p(i|i)$ are independent of
$i$ and give the
 probability of correct detection. The explicit result is
 $$
 \eqalign{
P_c=p(i|i)=&\Tr\left[B_{ii}^2\right]=\Tr\left[(G^{1/2})_{ii} \right]\cr
=&\frac{1}{m}\Tr\Bigl[\Bigl\{\sum_{k=0}^{m-1} D_k^{1/2}\Bigr\}^2\Bigr]\,.\cr}
\e(P25)
$$

Finally, we recall that the SRM  is optimal for GUS pure states, but not for GUS mixed states,
at least in
general.
In  particular, the sufficient condition for optimality given in
\bibl(Eldar3) fails in all our examples of application.


\vspace*{-5mm}

\Paragrafo(SN){Signal and Noise in Quantum Optical
          Communications}

      In this section we recall the quantum environment
for the signal and thermal noise in optical communications. The
correct settlement is provided by
the celebrated Glauber theory \bibl(Glauber), which represents signal
and noise in an infinite dimensional Hilbert space.

\vspace*{-3mm}

 \subsection{Representation of Coherent States }

The quantum model of a {\it coherent state} representing  a monochromatic
 electromagnetic radiation produced by a  laser is formulated in an
 infinite dimensional Hilbert space $\C(H)$ equipped with an orthonormal basis
 $|n\rangle, n=0,1,2,\ldots$, where $|n\rangle$  are called
{\it number eigenstates}. Each state $|n\rangle$ is said
to contain exactly $n$ photons. In this context the Glauber representation
 of a single  radiation mode is given by the ket
$$
\FB{|\gamma \rangle = e^{-\frac{1}{2}|\gamma|^2}
\sum_{n=0}^{\infty}{\frac{\gamma^n}{\sqrt{n!}}} |n\rangle}
\e(P2)
$$
where $\gamma$ is the complex envelope that specifies  the mode. Thus, for each
$\gamma \in\M(C)$ a coherent state (or Glauber state) is defined; in
particular, the state $|0\rangle$ obtained with $\gamma=0$ represents the
{\it ground state}.  The probability
of obtaining exactly $m$ photons   is
governed by the Poisson distribution
$
p(m|\gamma)= |\langle m|\gamma\rangle|^2
=\exp(-|\gamma|^2)\;|\gamma|^{2m}/{m !}
$
with mean $|\gamma|^2$. Hence,
$
N_\gamma=|\gamma|^2$ represents the {\it average number of photons} when the
system is in
  the coherent state $|\gamma \rangle$.
We recall that the Glauber states are not orthogonal, since
the inner product
of
two Glauber states   is given by
$$
\langle\alpha|\beta\rangle =
e^{-\frac{1}{2}(|\alpha|^2 + |\beta|^2 -2 \alpha^* \beta)}\;.
\e(P11)
$$



The representation  \e(P2) is only valid  when the
receiver observes a pure state with a known parameter $\gamma$, which in the
context of communications may be regarded as the {\it signal}. In the presence
of thermal (or background) noise the signal $\gamma$ becomes uncertain and must
be represented through a density operator. The Glauber theory
\bibl(Glauber)\bibl(Helstrom2)  states that the density operator is given by
$$\FB{
\BB(\rho)(\gamma)=\frac{1}{\pi\C(N)} \int_{\M(C)} \exp\Bigl(-\frac{|\alpha -
\gamma|^2}{\C(N)}\Bigr)\;|\alpha \rangle \langle \alpha| \, d\alpha}
\e(BB8)
$$
that is by a continuous mixture of coherent states. In \e(BB8) the
parameter $\C(N)$ represents the {\it  average number of photons}
associated with the thermal noise; it is given by
$
\C(N)=1/[\exp\left(h\nu/kT_0\right)-1]
$,
with $h$  Planck's constant, $k$  Boltzmann's constant, $\nu$  optical
frequency and $T_0$
 absolute temperature of the receiver.
Hence, the representation of ``signal plus noise''
 depends only on  the two parameters:
1) $\gamma\in\M(C)$, which determines the nominal coherent state
 $|\gamma\rangle$,
and 2) $\C(N)$ representing the average number of  noise photons.
 When $\C(N)=0$, that is in the absence of noise, relation
\e(BB8) degenerates into the pure state density operator
$\rho(\gamma)= |\gamma\rangle\langle\gamma|$.


\subsection{Discretization of the Density Operators}


An infinite matrix representation $||\rho_{mn}||$ of the density
 operator \e(BB8) is obtained in terms of
the orthonormal basis of the number eigenstates $|n\rangle$, namely
$\rho_{mn}=\langle m|\rho(\gamma)|n\rangle$, and the expression of the $m\,n$ entry
 is \bibl(Helstrom)
$$
\eqalign{\rho_{mn}(\gamma)=&(1- v)v^n \sqrt{\frac{m!}{n!}} \left(
\frac{\gamma^*}{\C(N)} \right)^{n-m}\cdot\cr
&\cdot e^{-(1- v)|\gamma|^2}\; L_{m}^{n-m}
 \left( - \frac{|\gamma|^2}{\C(N)(\C(N)+1)} \right)
       \cr}
\e(C20A)
$$
where $0\leq m\leq n $, $ \gamma\neq0$, $v=\C(N)/(1+\C(N))$ and $L_{m}^{n-m}(x)$ are the generalized Laguerre
polynomials. The entries  for $m> n$ are obtained by the symmetry
$\rho_{nm}(\gamma)=\rho_{mn}^*(\gamma)$. The
  matrix is infinite
dimensional and not diagonal.
The diagonal elements $\rho_{mm}(\gamma)$  give the probabilities
of obtaining exactly $m$ photons when the
quantum system is
in the noisy state $\rho(\gamma)$ \bibl(Helstrom). From \e(C20A)
we have
$$\eqalign{
p_L(m)=&\rho_{mm}(\gamma)\cr
       =&(1- v) v^m  \;
e^{-(1- v)N_\gamma}\;
L_{m} \Bigl( (1- v)^2N_\gamma/v \Bigr)\cr}
\e(BC45)
$$
which represents the {\it Laguerre distribution}
($L_{m}(x)=L_{m}^0(x)$ are the ordinary Laguerre
polynomials). The mean and the variance of distribution \e(BC45) are
$    N_\gamma+\C(N)$ and $
   N_\gamma+2N_\gamma\C(N)+\C(N)(\C(N)+1)$, respectively.
For the ground state $|\gamma\rangle= |0\rangle$  the above expressions
 degenerate. The matrix representation
 becomes diagonal, namely
$$
    \rho_{mn}(0)=\delta_{mn}(1-v)v^n
    \e(B7)
   $$
and the distribution becomes  {\it geometrical}:
$
   p_G(m)= \rho_{mm}(0)=(1-v)v^m    $.\Tabb(TQA4)6
The infinite dimension matrix  $||\rho_{mn}(\gamma)||,0\leq m,n<
\infty$ gives a correct representation of the density operator.
But, for the SRM, which is based on
\newpage

 \noindent eigendecompositions, we need a finite dimensional approximation by
 a truncation to $N_\epsilon$ terms.
For the choice of $N_\epsilon$ to get a given accuracy
we follow the  {\it quasi--unitary trace criterion}, which is
based on the fact that a  density operator has a unitary trace.
Then,  we choose $N_\epsilon$ as the smallest integer  such that
$$
\sum_{m=0}^{N_\epsilon-1}
              \rho_{mm}(\gamma)=\sum_{m=0}^{N_\epsilon-1} p_L(m)\geq 1-\epsilon
$$
where  $\epsilon$ is the required accuracy. Thus, for a given $\epsilon$,
$N_\epsilon$ can be evaluated using the Laguerre distribution \e(BC45).

\subsection{Factorization of the Density Operators}

Once established the finite $N_\epsilon\times N_\epsilon$ approximation
 of the density operators, for the SRM we need
  a factorization of the form
$
  \rho(\alpha) =\gamma(\alpha)\gamma^*(\alpha)
  $
  for a convenient matrix $\gamma(\alpha)$, which we call state factor.
This is obtained
from the eigendecomposition of $\rho(\alpha)$, namely
$$
\rho(\alpha)=\sum_{i=1}^r\lambda_i^2\,|u_i\rangle\langle u_i|
=U_r\Lambda_r^2 U_r^*
$$
where $r$ is the rank of $\rho(\alpha)$, $U_r$  is $N_\epsilon\times r$ and
collects the eigenvectors $|u_i\rangle$
corresponding to the $r$ positive eigenvalues $\lambda_i^2$, which
are assumed in a decreasing order, and  $\Lambda_r^2$ is
$r\times r$ diagonal collecting the $\lambda_i^2$.
Hence,
$
\gamma(\alpha)=U_r\,\Lambda_r
$
is a correct factor of $\rho(\alpha)$. (For $\alpha=0$ (ground state) the factorization
 is immediate since $\rho(0)$ is diagonal and from \e(B7)
we find
$
\gamma(0)
  =\sqrt{\rho(0)}=||\delta_{mn}\sqrt{(1-v)v^n} ||
$.)

A critical point in the numerical evaluation is the choice of the rank $r$,
 given by the number
of the numerically relevant positive eigenvalues.  To clarify
 the problem
 we develop a specific case:
$
 \alpha=\sqrt5\vl N_\alpha=5\vl \C(N)=0.1\vl\epsilon=10^{-5}\q\arr\q
 N_\epsilon=20
$. Now, in theory $\rho(\alpha)$ has
 a full rank $r=N_\epsilon$, as we can  see from the list of its eigenvalues
 obtained with a great accuracy
\begin{footnotesize}
$$
\eqalign{
&0.150285\vl0.00231095\vl0.0000353779\vl
          5.20725 10^{-7}  \vl7.24874  10^{-9}\cr
&9.45157 10^{-11}\vl1.14603 10^{-12} \vl\ldots\vl
  1.3445 10^{-19}   \vl-4.13564 10^{-20}\cr
&\!\!-3.10867 10^{-21}   \vl
 2.32186 10^{-21}   \vl-1.37631 10^{-22}   \vl3.01775 10^{-25}\cr
 }
$$
\end{footnotesize}%
but  in practice we can limit to take only the first 3 eigenvalues,
neglecting the remaining, which means that
 we assume as a ``practical'' rank $r=3$. As a check, the reconstruction
 of $\rho(\alpha)$ obtained in such a way assures an accuracy $<10^{-7}$.
 To find the ``practical'' rank in general we consider the reconstruction
 \newpage
\noindent error
$\Delta\rho=\rho-\gamma_r\gamma^*_r$,
where  the factor $\gamma_r$ is obtained by considering only $r$ eigenvalues.
Then, we can  evaluate the
 maximum error or the mean square error
(m.s.e.) as a function of $r$ and we
 choose $r=N_\nu$ to achieve a given accuracy
$\nu$.


In \Tabb(TQA4)0 we give a collection  of $N_\epsilon$ and $N_\nu$
for some values of $N_\gamma$ and $\C(N)$, obtained with the accuracies
$\epsilon=\nu=10^{-5}$.  $N_\nu$ was obtained  considering the m.s.e.





\Paragrafo(QAM){Application to  QAM Modulation}

The $m$--QAM constellation is defined starting from the auxiliary alphabet
$
\C(A)_L=\{-(L-1)+2(i-1)|\;i=1,2,\ldots,L\}$ with $ L=2,3,\ldots$
and is given by the $m$ Glauber states
$$
|\gamma_{uv}\rangle=|\Delta(u+iv)\rangle\vq u,v\in\C(A)_L
\e(C33)
$$
with $m=L^2$. This constellation has not
the GUS and therefore the SRM must be applied in the general form.
In \e(C33) $\Delta$ is a scale factor, which  determines the
average number of signal photons, specifically
$$
N_s=\frac{2}{3}(L^2-1)\Delta^2=\frac{2}{3}(m-1)\Delta^2\;.
\e(Z34)
$$
For instance, for the 16--QAM we find $N_s=10 \Delta^2$.

%\newpage
In the case of pure states the first step is the evaluation
of the Gram matrix $G$, whose elements are given by the inner products%
\footnote{$G$ depends on the four indexes
        $u,v,u',v'$, but it can be arranged as an ordinary matrix using
     the lexicographic order
       for the indexes.}
$$
\eqalign{\langle\gamma_{uv}|&\gamma_{u'v'}\rangle=
       \langle\Delta(u+iv)|\Delta(u'+iv')\rangle\cr
       &=\exp\{-\fract{1}{2}
\Delta^2[(u'-u)^2+(v'-v)^2-2i(u'v-v'u)]\}\cr
       &\hskip25mm  u,v,u',v'\in\C(A)_L\;.\cr}
$$
Then, the eigendecomposition $G=V\Lambda_GV^*$, the evaluation of $G^{1/2}$
and of the probabilities can be carried out without approximation and
with a low
computational complexity since the dimensions involved are
 only $m\times m$ \bibl(Kato1999).

\subsection{Application of SRM in the Presence of Noise}
In the presence of thermal noise
the only problem is the management of approximations since
the density operators must be approximated by  finite--dimensional matrices,
as discussed in Section IV. In the QAM format the average number of photons
$N_\gamma=|(u+iv)\Delta|^2$, is not uniform over the constellation,
 varying from $N_\gamma=2\Delta^2$ for
the inner symbols to $N_\gamma=2(L-1)^2\Delta^2$ for the corner symbols.
The reduced dimensions of the Hilbert space $n=N_\epsilon$ must be chosen
considering the maximum $N_{\gamma,\hbf{max}}=2(L-1)^2\Delta^2$.
Then, assuming  $N_s$ as fundamental parameter, for the choice of $N_\epsilon$
we have to consider that
$$
N_{\gamma\hbf{max}}=3[(L-1)^2/(L^2-1)] \,N_s=3[(L-1)/(L+1)]\,N_s\;.
$$
For instance, for  16--QAM we find $N_{\gamma\hbf{max}}=1.8N_s$.


We sketch an example to illustrate the dimensions involved in the 16--QAM.
With $N_s=4$ and $\C(N)=0.1$
we find $N_{\gamma\hbf{max}}=7.2$ and we choose $N_\epsilon=40$ assuring an
accuracy
$\epsilon=10^{-7}$. The dimensions of the $\rho_i$ are $40\times40$
and they are factored into matrices $\gamma_i$
of dimensions
 $40\times8$. The dimensions of $\Gamma$, $T$ and $G$ are
$40\times128$, $40\times40$, $128\times128$, respectively. So, it is
more efficient  to compute $T^{-1/2}$ rather than $G^{\pm1/2}$. With the above
choices we find the following diagonal transition probabilities:
 0.875749 for inner states,
 0.916501 for side states,
 0.947767 for corner states,
and the average error probability is
$P_e=0.08587$.


The SRM approach has been applied systematically to evaluate the error probability
$P_e$
in the 16--QAM systems following the steps outlined above. The results
are  illustrated in \Figg(QA117)0, where $P_e$ is plotted
versus the average number of photons per symbol $N_s$ for some values
of the thermal noise parameter $\C(N)$. In particular, the curve for $\C(N)=0$,
which refers to the absence of thermal noise, was checked with
the results obtained with pure states and a perfect agreement has been found.
To assure an overall accuracy of $\epsilon=10^{-7}$, the dimensions of the
Hilbert space have been set to the value
$n=N_\epsilon=130$. %\Figg(QA116)2

In \fig(QA117) the performance of the SRM quantum detector is also
compared with the performance of the classical homodyne detector, for which
a Gaussian additive model with SRN=$4N_s/(1+2\C(N))$ results.%
\footnote{In
Kato {\it et al.} \bibl(Kato1999) an analogous comparison is made
with heterodyne detector.} %
In the absence of thermal noise
 an improvement of about 3 dB over homodyne detection is confirmed. As it was
 expected, this improvement rapidly reduces as thermal noise increases.
(For a comparison with optimum detection see the end of Section VI).


\Figg(QA117)2


\Paragrafo(PSK){Application to the PSK Modulation}

The constellation of a coherent PSK modulation format is given by
the Glauber states
$
\ket(\gamma_i)=\ket(\gamma_0 W_m^i),i=0,\ldots,m-1
$,
where, without loss of generality, we  assume that $\gamma_0$ is
real positive. This is a GUS constellation with initial state
$\ket(\gamma_0)$ and generating operator
$$
S=\sum_{n=0}^\infty W_m^n\kb(n,n) \;.
\e(P34A)
$$
%\Figg(QA116)2

With pure states the performance evaluation  starts from
the inner products $G_{0s}=\langle\gamma_0|\gamma_s\rangle$,
 which can be obtained from \e(P11), namely
$$
G_{0s} =\exp[-\gamma_0^2(1-W_{m}^{s})] \vq s=0,1,\ldots,m-1 \;.
\e(D21)
$$
Then, the eigenvalues of the Gram matrix are obtained as the DFT of $G_{0s}$
$$
D_k = \sum_{s=0}^{m-1}G_{0s}W_{m}^{-ks}
\e(D22)
$$
Finally, the minimum error probability is
$$
P_e = 1-\frac{1}{m^2}\Bigl(\sum_{k=0}^{m-1}\sqrt{D_k}\Bigl)^2\;.
\e(D26)
$$

The above expressions are obtained without numerical approximations. $P_e$
 is a function of the alphabet size $m$ and of the
parameter $\gamma_0$, whose square
$N_s=\gamma_0^2$ gives the {\it average number of photons per symbol}.

\vspace*{-3mm}

\subsection{Application of the SRM-GUS in the Presence of Noise}

The $m$ Glauber density operators obtained with a PSK constellation
verify the GUS with generating operator $S$ given by \e(P34A), which has
infinite dimensions. In the SRM $S$ must be reduced to a finite dimension
$n$ and  then, in matrix form, it becomes
$$
S=\diag[W_m^k,k=0,1,\ldots,n-1]\;.
$$
Its eigendecomposition $S=Y\,\Lambda\,Y^*$ is trivial with $Y=I_n$
and $\Lambda=S$, and the matrices $L_k$ are given by
$$
   L_k=m\,\diag[\delta_{k,i\mod m},i=0,1,\ldots,n-1]
$$

 Now,
  for a given $n$, $N_s=\gamma_0^2$ and $\C(N)$,
the application of the SRM--GUS proceeds as follows:
 1) evaluate the reference density operator $\rho_0=\rho_0(\gamma_0)$
      from \e(C20A);
 2) find the factor $\gamma_0$ of   $\rho_0$;
 3) evaluate the blocks $D_k=\gamma_0^*L_k\gamma_0$
      and find the square roots $D^{1/2}_k$ by eigendecomposition;
 4) evaluate the blocks $B_{ii}=(G^{1/2})_{ii}$ from \ee(P25)a;      5) evaluate $P_c$ from \e(P25).


\ET We give a detailed example of calculation in the case of small
dimensions (for reason of space). We consider the 4--PSK with $N_s=1$,
$\C(N)=0.1$ and $N_\epsilon=8$, which assures an accuracy of $\epsilon=10^{-5}$.
The reference density operator is the $8\times8$ matrix

\begin{tiny}
$$
\hbs{$\rho_0=$}\qmatrix{0.366 & 0.333 & 0.214 & 0.112 & 0.051 & 0.021 & 0.008 & 0.003 \cr\VS0
0.333 & 0.336 & 0.237 & 0.136 & 0.067 & 0.029 & 0.012 & 0.004 \cr\VS0
0.214 & 0.237 & 0.183 & 0.114 & 0.060 & 0.028 & 0.012 & 0.005 \cr\VS0
0.112 & 0.136 & 0.114 & 0.076 & 0.044 & 0.022 & 0.010 & 0.004 \cr\VS0
0.051 & 0.067 & 0.060 & 0.044 & 0.027 & 0.014 & 0.007 & 0.003 \cr\VS0
0.021 & 0.029 & 0.028 & 0.022 & 0.014 & 0.008 & 0.004 & 0.002 \cr\VS0
0.008 & 0.012 & 0.012 & 0.010 & 0.007 & 0.004 & 0.002 & 0.001 \cr\VS0
0.003 & 0.004 & 0.005 & 0.004 & 0.003 & 0.002 & 0.001 & 0.001\cr}
 $$
 \end{tiny}
Its practical rank is 5.
From the  eigendecomposition of $\rho_0$ we obtain the $8\times 5$ factor
\begin{tiny}
$$
\hbs{$\gamma_{0}=$}\qmatrix{-0.289 & 0.087 & -0.019 & -0.003 & 0.000 \cr\VS0
-0.289 & 0.000 & 0.019 & 0.006 & 0.001 \cr\VS0
-0.204 & -0.062 & 0.013 & -0.002 & -0.002 \cr\VS0
-0.118 & -0.071 & -0.008 & -0.005 & 0.000 \cr\VS0
-0.059 & -0.053 & -0.019 & 0.000 & 0.001 \cr\VS0
-0.026 & -0.032 & -0.019 & 0.004 & 0.000 \cr\VS0
-0.011 & -0.016 & -0.013 & 0.006 & -0.001 \cr\VS0
-0.004 & -0.007 & -0.008 & 0.005 & -0.002\cr}
 $$
\end{tiny} The matrices $L_k$ are
\begin{tiny}
 $$
\hbs{$L_0=$}\qmatrix{4 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 4 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\cr}
 \qq
\hbs{$L_1=$}\qmatrix{0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 4 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 4 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \cr\VS0
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\cr}\q\dots
 $$
\end{tiny} Then the evaluation of $D_k$ and its square
 root, e.g. for
$k=0$, gives
\begin{tiny}
$$\eqalign{
\hbs{$D_{0}=$}&\qmatrix{0.348 & -0.088 & 0.026 & 0.004 & 0.000 \cr\VS0
-0.088 & 0.042 & -0.002 & -0.001 & 0.000 \cr\VS0
0.026 & -0.002 & 0.003 & 0.000 & 0.000 \cr\VS0
0.004 & -0.001 & 0.000 & 0.000 & 0.000 \cr\VS0
0.000 & 0.000 & 0.000 & 0.000 & 0.000\cr}\cr
\hbs{$D_0^{1/2}=$}&\qmatrix{0.576 & -0.121 & 0.048 & 0.006 & 0.000 \cr\VS0
-0.121 & 0.164 & 0.020 & -0.002 & -0.003 \cr\VS0
0.048 & 0.020 & 0.010 & 0.000 & -0.001 \cr\VS0
0.006 & -0.002 & 0.000 & 0.000 & 0.000 \cr\VS0
0.000 & -0.003 & -0.001 & 0.000 & 0.000\cr}\cr}
 $$
 \end{tiny} Finally, the  probabilities
 are
\begin{tiny}
$$\eqalign{
&\hbs{$p_c=$}\qmatrix{0.80703 & 0.08622 & 0.02034 & 0.08622 \cr\VS0
0.08622 & 0.80703 & 0.08622 & 0.02034 \cr\VS0
0.02034 & 0.08622 & 0.80703 & 0.08622 \cr\VS0
0.08622 & 0.02034 & 0.08622 & 0.80703\cr}\cr\VS3
&\hbf{$P_c=0.80703\qq P_e=0.19297\;.$}\cr}
 $$
\end{tiny}

\vspace*{-3mm}

\subsection{Performance of 4--PSK and 8--PSK}

The SRM--GUS approach has been applied to evaluate the error probability
$P_e$
in 4--PSK and 8--PSK systems following the steps outlined above. The results
are  illustrated in \Fig(QA310) and in \Fig(QA114), where $P_e$ is plotted
versus the average number of photons per symbol $N_s$ for some values
of the thermal noise parameter $\C(N)$. In particular, the curve for $\C(N)=0$,
which refers to the absence of thermal noise, was checked with
the results obtained with pure states (see \e(D26)) and a perfect agreement has been found.
To assure an overall accuracy of $\epsilon=10^{-5}$, the reference
density operator $\rho_0$ was approximated with a matrix of size
$N_\epsilon=145$ with a rank running from 1 to 48 in dependence of $\C(N)$.



In \fig(QA310) and \fig(QA114) the PSK quantum detection is compared with
homodyne counterpart. Remarks similar to that made for 16--QAM
can be repeated.\Figg(QA224)6

\subsection{SRM vs Optimal Measurement}

For mixed states, the SRM approach is not optimal, at least in general, so that
a comparison with the optimal performances is adequate. As mentioned above,
the maximum probability of correct detection is the maximum of
$\sum_{i=0}^{m-1}\Tr(q_i\rho_i\Pi_i)
$
under the constraints that the $\Pi_i$ are PSD and resolve the identity
$I_{\C(H)}$ or, equivalently \bibl(Holevo), the minimum of $\Tr(Y)$ under the
constraint that the operators $Y-q_i\rho_i$ are PSD. This is a problem of convex
semidefinite programming. The numerical evaluation of the optimum for the
applications considered in the paper have been performed by Matlab with the LMI
(Linear Matrix Inequality) Toolbox. A comparison is presented in \Figg(QA224)0 for
the 2--PSK and 4--PSK
 systems and shows that the SRM exhibits an error
probability about 30\% greater than the optimum detector. Since similar results
hold true also for 8--PSK and 16--QAM, we conclude that SRM is ``pretty good''
also in the presence of thermal noise.
\ev{Remark} For the 2--PSK (as for any other binary format)
                            the exact evaluation can be carried out using Helstrom's
                theory (see \bibl(Helstrom2)). This possibility was used to check
                the results obtained with the Matlab LMI toolbox.

\Paragrafo(CON){Conclusions}

We calculated the error probability of QAM and PSK quantum data
communication system in the presence of thermal noise with
quantum detection based on the SRM technique. The main novelty of
the paper lies in the  performance evaluation  of
quantum data transmission system affected by thermal noise, not
necessarily in a small amount. The lack of results in the
literature about this topic is surely due to the difficulties of
numerical computation of optimal detection. The extension of the
SRM approach to mixed states by Eldar {\it et al.} \bibl(Eldar3) allowed
us to develop such computations with a relatively limited amount
of numerical complexity.


Comparisons  made with the performance of
classical homodyne detection give results similar to
that for OOK and BPSK schemes and evidence the superiority
of the quantum detection also in the presence of thermal noise.
A comparison of the SRM with the optimal detection performance,
evaluated by a convex semidefinite programming package, shows
only a moderate impairment, so that the obtained results can
be considered a very good approximation of the optimal
performances.

The results of the application of the SRM to geometrically
uniform symmetric states will enable one to consider other
quantum modulation schemes, both in absence and in presence of
thermal noise. In particular, pulse position modulation (PPM) %\newpage
 has
recently been considered \bibl(JPLbook) for possible applications
 to deep
space quantum communications.\newpage However, further problems of
computational complexity arise, owing to the fact that the
natural model for the PPM scheme is the tensorial product of
Hilbert spaces. Our research on the topic is in progress.%\newpage


\subsection*{Acknowledgment}
The authors would like to thank Roberto Corvaja for his helpful
support and criticism.

